Rethinking Node Representation Interpretation through Relation Coherence

Understanding node representations in graph-based models is crucial for uncovering biases ,diagnosing errors, and building trust in model decisions. However, previous work on explainable AI for node representations has primarily emphasized explanations (reasons for model predictions) rather than interpretations (mapping representations to understandable concepts). Furthermore, the limited research that focuses on interpretation lacks validation, and thus the reliability of such methods is unclear. We address this gap by proposing a novel interpretation method-Node Coherence Rate for Representation Interpretation (NCI)-which quantifies how well different node relations are captured in node representations. We also propose a novel method (IME) to evaluate the accuracy of different interpretation methods. Our experimental results demonstrate that NCI reduces the error of the previous best approach by an average of 39%. We then apply NCI to derive insights about the node representations produced by several graph-based methods and assess their quality in unsupervised settings.

==> fig/data_stats.tex <==
\begin{small}
\begin{table}[t]
\caption{Data Statistics.}
\vspace{-4mm}
\label{tab:dataset}
\begin{center}
\begin{tabular}{lrrrr}
\hline
Dataset & Node & Edge & Node Class & Node Attr. \\
\hline
Cora & 2708 & 10556 & 7 & 1433 \\
CiteSeer & 3327 & 9104 & 6 & 3703 \\
Brazil & 131 & 1074 & 4 & - \\
USA & 1190 & 13599 & 4 & - \\
Computers & 13752 & 491722 & 10 & 767 \\
Photo & 7650 & 238162 & 8 & 745 \\
\hline
\end{tabular}
\vspace{-4mm}
\end{center}
\end{table}
\end{small}

==> fig/framework.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/framework.jpg}
  \caption{Testing framework for Node Coherence Test.}
  \vspace{4mm}
  \label{fig:framework}
\end{figure}

==> fig/svd_dim.tex <==

\begin{figure}[t]
  \centering
  \vspace{-5mm}
  \includegraphics[width=0.65\linewidth]{fig/usa_svd_dim.pdf}
  \vspace{-1mm}
  \caption{When the embedding has noise ($d\leq 512$), our Node Coherence Test has better interpretation accuracy (MRR) compared to other representation interpretation methods.}
  \vspace{-4mm}
  \label{fig:svd_dim}
\end{figure}
